LiSA: Lifelong Safety Adaptation via Conservative Policy Induction

As AI agents move from chat interfaces to systems that read private data, call tools, and execute multi-step workflows, guardrails become a last line of defense against concrete deployment harms. In these settings, guardrail failures are no longer merely answer-quality errors: they can leak secrets, authorize unsafe actions, or block legitimate work. The hardest failures are often contextual: whether an action is acceptable depends on local privacy norms, organizational policies, and user expectations that resist pre-deployment specification. This creates a practical gap: guardrails must adapt to their own operating environments, yet deployment feedback is typically limited to sparse, noisy user-reported failures, and repeated fine-tuning is often impractical. To address this gap, we propose LiSA (Lifelong Safety Adaptation), a conservative policy induction framework that improves a fixed base guardrail through structured memory. LiSA converts occasional failures into reusable policy abstractions so that sparse reports can generalize beyond individual cases, adds conflict-aware local rules to prevent overgeneralization in mixed-label contexts, and applies evidence-aware confidence gating via a posterior lower bound, so that memory reuse scales with accumulated evidence rather than empirical accuracy alone. Across PrivacyLens+, ConFaide+, and AgentHarm, LiSA consistently outperforms strong memory-based baselines under sparse feedback, remains robust under noisy user feedback even at 20% label-flip rates, and pushes the latency--performance frontier beyond backbone model scaling. Ultimately, LiSA offers a practical path to secure AI agents against the unpredictable long tail of real-world edge risks.

==> table/main_results.tex <==

% Google Brand Colors Definition
\definecolor{GoogleBlue}{HTML}{4285F4}
\definecolor{GoogleRed}{HTML}{EA4335}
\definecolor{GoogleYellow}{HTML}{FBBC05}
\definecolor{GoogleGreen}{HTML}{34A853}

% Pastel Backgrounds for Table
\definecolor{bgGray}{gray}{0.95}
\definecolor{bgYellow}{HTML}{FEF7E0} % Light version of Google Yellow
\definecolor{bgRed}{HTML}{FCE8E6}    % Light version of Google Red
\definecolor{bgGreen}{HTML}{E6F4EA}  % Light version of Google Green
\definecolor{bgBlue}{HTML}{E8F0FE}   % Light version of Google Blue

\begin{table*}[t!]
\caption{Performance comparison of different defense methods on AgentDojo datasets. 
Metrics include Benign Utility (BU $\uparrow$), Benign Latency (BL $\downarrow$), Utility under Attack (UA $\uparrow$), Latency under Attack (LA $\downarrow$), and Attack Success Rate (ASR $\downarrow$).
Defense categories are color-coded: 
\colorbox{bgGray}{No Defense}, 
\colorbox{bgYellow}{Prompting}, 
\colorbox{bgRed}{Trained Classifier}, 
\colorbox{bgGreen}{System-based Defenses}, and 
\colorbox{bgBlue}{Our Proposed Method (CausalArmor)}.}
\label{table-overall results}
\centering
\resizebox{0.96\textwidth}{!}{
\begin{tblr}{
  width=\textwidth,
  colspec={c l | c c | c c c | c c c | c c c },
  % --- Row Coloring based on Categories (Re-indexed) ---
  % Gemini-2.5-flash (Rows 3-10)
  row{3}={bg=bgGray},          % No Defense
  row{4}={bg=bgYellow},        % Prompting (Repeat Prompt ONLY now)
  row{5-6}={bg=bgRed},         % Classification (DeBERTa, PiGuard)
  row{7-9}={bg=bgGreen},       % System (DRIFT, Melon, PromptArmor)
  row{10}={bg=bgBlue},         % CausalArmor
  % Claude-4-Sonnet (Rows 11-18)
  row{11}={bg=bgGray},
  row{12}={bg=bgYellow},
  row{13-14}={bg=bgRed},
  row{15-17}={bg=bgGreen},
  row{18}={bg=bgBlue},
  % Gemini-3-pro (Rows 19-25)
  row{19}={bg=bgGray},
  row{20}={bg=bgYellow},
  row{21-22}={bg=bgRed},
  row{23-24}={bg=bgGreen},
  row{25}={bg=bgBlue},
  % Header Styling
  row{1-2}={font=\bfseries, bg=white},
  column{1}={font=\bfseries, bg=white},
  % Borders (Adjusted indices)
  hline{1,Z}={1.5pt},
  hline{2}={1pt},
  hline{3}={1pt},   % After headers
  hline{11}={1pt},  % Between Gemini-2.5 and Claude (Previously 12)
  hline{19}={1pt},  % Between Claude and Gemini-3 (Previously 21)
  vline{2}={1pt},
  vline{3,5,8,11}={0.5pt},
  cell{1}{1}={c}, cell{1}{2}={c}, cell{1}{3}={c},
  cell{1}{5}={c}, cell{1}{8}={c}, cell{1}{11}={c},
}
  % Header Row 1
  \SetCell[r=2]{c} \textbf{Backbone Model} & \SetCell[r=2]{c} \textbf{Defense Method}
  & \SetCell[c=2]{c} \textbf{No Attack} & & \SetCell[c=3]{c} \textbf{Important Instructions} & & & \SetCell[c=3]{c} \textbf{New Attack 1} & & & \SetCell[c=3]{c} \textbf{New Attack 2} & & \\
   
  % Header Row 2
  & & \textbf{BU $\uparrow$} & \textbf{BL $\downarrow$} & \textbf{UA $\uparrow$} & \textbf{LA $\downarrow$} & \textbf{ASR $\downarrow$} & \textbf{UA $\uparrow$} & \textbf{LA $\downarrow$} & \textbf{ASR $\downarrow$} & \textbf{UA $\uparrow$} & \textbf{LA $\downarrow$} & \textbf{ASR $\downarrow$} \\

  % --- Gemini-2.5-Flash Block (Row count reduced from 9 to 8) ---
  \SetCell[r=8]{c} \textbf{Gemini-2.5-Flash} 
  & No Defense & 53.61 & 1.00 & 32.46 & 1.00 & 32.47 & 51.59 & 1.00 & 12.01 & 47.48 & 1.00 & 7.06 \\
  & Repeat Prompt & 64.95 & 1.15 & 41.41 & 1.15 & 35.93 & 50.01 & 1.15 & 8.51 & 51.53 & 1.14 & 7.38 \\
  % Spotlight Removed
  & DeBERTa Detector & 30.93 & 1.16 & 16.75 & 1.24 & 7.27 & 33.62 & 1.20 & 4.21 & 28.35 & 1.24 & 4.11 \\
  & PiGuard & 32.99 & 1.22 & 8.01 & 1.28 & 1.05 & 8.43 & 1.29 & 0.42 & 10.96 & 1.30 & 0.0 \\
  & DRIFT & 50.58 & 4.67 & 16.87 & 6.75 & 4.99 & 36.38 & 5.58 & 2.48 & 42.44 & 5.25 & 1.25 \\
  & Melon & 49.48 & 2.21 & 13.8 & 2.83 & \textbf{0.53} & 28.72 & 3.12 & \textbf{0.21} & 30.98 & 2.67 & \textbf{1.05} \\
  & PromptArmor & 41.24 & 2.44 & 41.82 & 2.65 & \textbf{0.63} & 50.32 & 2.50 & \textbf{0.0} & 51.74 & 2.71 & \textbf{0.24} \\
  & CausalArmor & \textbf{56.26} & \textbf{1.30} & \textbf{50.90} & \textbf{1.96} & \textbf{0.62} & \textbf{54.64} & \textbf{1.78} & \textbf{0.42} & \textbf{52.53} & \textbf{1.81} & \textbf{0.40} \\

  % --- Claude-4-Sonnet Block (Row count reduced from 9 to 8) ---
  \SetCell[r=8]{c} \textbf{Claude-4-Sonnet} 
  & No Defense & 89.44 & 1.00 & 83.98 & 1.00 & 2.32 & 85.77 & 1.00 & 3.37 & 81.77 & 1.00 & 18.97 \\
  & Repeat Prompt & 67.01 & 1.20 & 69.02 & 1.18 & 0.84 & 68.60 & 1.21 & 1.26 & 67.33 & 1.24 & 7.27 \\
  % Spotlight Removed
  & DeBERTa Detector & 55.67 & 1.10 & 49.63 & 1.12 & 1.37 & 62.80 & 1.11 & 1.79 & 55.32 & 1.14 & 6.53 \\
  & PiGuard & 62.89 & 1.15 & 31.30 & 1.16 & 0.63 & 25.40 & 1.15 & 0.0 & 27.92 & 1.20 & 0.42 \\
  & DRIFT & 72.27 & 5.43 & 66.92 & 6.63 & 0.82 & 65.31 & 6.38 & 0.63 & 55.53 & 7.59 & 2.48 \\
  & Melon & 74.29 & 2.31 & 41.41 & 2.41 & \textbf{0.21} & 41.84 & 2.48 & \textbf{0.21} & 42.47 & 2.72 & \textbf{0.0} \\
  & PromptArmor & 74.23 & 2.20 & 74.08 & 2.44 & \textbf{0.0} & 74.29 & 2.40 & 0.0 & 75.87 & 2.66 & 0.0 \\
  & CausalArmor & \textbf{82.47} & \textbf{1.27} & \textbf{83.67} & \textbf{1.54} & \textbf{0.0} & \textbf{83.67} & \textbf{1.56} & \textbf{0.11} & \textbf{83.03} & \textbf{1.70} & \textbf{0.46} \\

  % --- Gemini-3-pro Block (Row count reduced from 8 to 7) ---
  \SetCell[r=7]{c} \textbf{Gemini-3-Pro} 
  & No Defense & 92.78 & 1.00 & 90.41 & 1.00 & 5.06 & 89.88 & 1.00 & 5.69 & 89.78 & 1.00 & 8.85 \\
  & Repeat Prompt & 92.78 & 1.16 & 89.99 & 1.18 & 2.85 & 89.44 & 1.17 & 4.11 & 89.36 & 1.21 & 6.11 \\
  % Spotlight Removed
  & DeBERTa Detector & 58.76 & 1.04 & 55.43 & 2.06 & 1.05 & 56.31 & 1.05 & 3.37 & 56.80 & 1.06 & 6.11 \\
  & PiGuard & 64.95 & 1.06 & 31.19 & 1.06 & 0.63 & 25.92 & 1.06 & 0.63 & 29.92 & 1.07 & 0.84 \\
  & DRIFT & 81.05 & 5.82 & 70.65 & 6.44 & 3.85 & 71.45 & 6.61 & 3.65 & 66.68 & 6.53 & 4.24 \\
  & PromptArmor & 77.32 & 1.78 & 83.35 & 1.98 & \textbf{0.11} & 83.67 & 2.01 & 0.11 & 83.77 & 2.05 & 0.32 \\
  & CausalArmor & \textbf{86.60} & \textbf{1.22} & \textbf{87.14} & \textbf{1.44} & \textbf{0.11} & \textbf{88.09} & \textbf{1.43} & \textbf{0.11} & \textbf{87.88} & \textbf{1.53} & \textbf{0.0} \\

\end{tblr}
\label{tab:main_results}
}
\end{table*}

